Bridging the Gap Between Promise and Performance for Microscaling FP4 Quantization

The recent hardware-accelerated microscaling 4-bit floating-point formats such as MXFP4 and NVFP4, supported on NVIDIA and AMD GPUs, promise to revolutionize large language model (LLM) inference. Yet, their practical benefits remain unproven. We present the first comprehensive study of MXFP4 and NVFP4 for post-training quantization, revealing gaps between their promise and real-world performance. Our analysis shows that state-of-the-art methods struggle with FP4, due to two key issues: (1) NVFP4's small group size provably neutralizes traditional outlier mitigation techniques; (2) MXFP4's power-of-two scale quantization severely degrades accuracy due to high induced error. To bridge this gap, we introduce Micro-Rotated-GPTQ (MR-GPTQ), a variant of the classic GPTQ quantization algorithm that tailors the quantization process to FP4's unique properties, by using block-wise Hadamard transforms and format-specific optimizations. We support our proposal with a set of high-performance GPU kernels that enable the MR-GPTQ format with negligible overhead, by rotation fusion into the weights, and fast online computation of the activations. This leads to speedups vs. FP16 of up to 3.6x layer-wise, and 2.2x end-to-end on NVIDIA B200, and of 6x layer-wise and 4x end-to-end on RTX5090. Our extensive empirical evaluation demonstrates that MR-GPTQ matches or outperforms state-of-the-art accuracy, significantly boosting MXFP4, to the point where it can near the accuracy that of NVFP4. We conclude that, while FP4 is not an automatic upgrade over INT4, format-specialized methods like MR-GPTQ can unlock a new frontier of accuracy-performance trade-offs.

==> transformations.tex <==

In this section, we ablate using different transformations during join-quantization of \textbf{LLaMa3-8B} model with both NvFP4 and MXFP4. The list of transformations are: 


\begin{itemize}
\item Non-Trainable Transformations:
\begin{itemize}
    \item Deterministic Hadamard transformation
    \item DCT and DST
    \item FastFood Transformations
\end{itemize}
\item Trainable Transformations:
\begin{itemize}
    \item SpinQuant 
    \item FlatQuant
\end{itemize}
\end{itemize}


For non-trainable transformations, we try different block sizes (including 16, 32, 64, 128, and 256) for both NvFP4 and MXFP4 formats. We always quantize the weights with GPTQ (without sweeping over the parameters), and evaluate over \textbf{hellaswag}, \textbf{winogrande}, \textbf{PiQA}, \textbf{Arc-C}, and \textbf{Arc-E}. This will be 10 different combinations of the experiments for non-trainable transformations (and 2 for trainable transformations).



%
%\begin{table}
%    \centering
%
%    
%
%\begin{tabular}{c|c|ccccc}
%
%
%
%\multirow{2}{*}{Format} &\multirow{2}{*}{Transformation}  &   \multicolumn{5}{c}{Transformation Size}   \\ \cmidrule{3-7}
% &    & \texttt{16}   & \texttt{32}  & \texttt{64} & \texttt{128} & \texttt{256} \\ \toprule 
%\multirow{5}{*}{NvFP4} &  DCT  & 0.70069    &  0.70264   &  0.69393 &0.69815&  0.69981 \\ 
%                       &  DST  &  0.69063   & 0.70058  &  0.70323 & 0.70132  & 0.70269  \\ 
%                       &  GSR  &   0.70285  &  0.70021  &  0.70124 & 0.71272  &  0.70159 \\ 
%                       &  FastFood  &   NaN  &  0.35452  & 0.35531  & 0.35873  & 0.35586  \\  
%                       &  Hadamard  &  0.6987   &  0.6972  &  0.6923 & 0.6983  & NaN  \\  \midrule
%                       
%\multirow{5}{*}{MXFP4} &  DCT  &   0.6912  &  0.67691  &  0.68909 &  0.68309 & 0.68581  \\ 
%                       &  DST  &   0.69289  &  0.64809  &  0.6724 &  0.68779 &  0.68771 \\ 
%                       &  GSR  &  0.70285   &  0.70021  & 0.70124  & 0.7022  & 0.68986  \\
%                       &  FastFood  &  0.36411   & 0.35797   & 0.35812  & 0.35861  & NaN  \\ 
%                       &  Hadamard  &  0.6913   & 0.6923   &  0.7000 & 0.7046  &  0.6953 \\  
%
%\bottomrule
%
%\end{tabular}
%
%
%
%
%\caption{Zero-shot accuracy (averaged over 5 different tasks) of using different non-trainable transformations with different sizes on LLaMa3-8B model. The baseline model has 0.7274 accuracy.}
%
%
%
%\end{table}



\begin{table}
    \centering
\begin{tabular}{c|c|ccccc}
\multirow{2}{*}{Format} & \multirow{2}{*}{Transformation} & \multicolumn{5}{c}{Transformation Size} \\ \cmidrule{3-7}
 & & \texttt{16} & \texttt{32} & \texttt{64} & \texttt{128} & \texttt{256} \\ \toprule 
\multirow{5}{*}{NVFP4}     & Hadamard & 0.7004 & 0.6988 & 0.70201 & 0.70557 & NaN \\  
& DCT & 0.70826 & 0.69057 & 0.69518 & 0.7046 & 0.69604 \\ 
                       & DST & 0.69534 & 0.69479 &0.70896  & 0.70189 &0.69869  \\ 
                       & GSR & 0.70806  & 0.7053 &  0.70034 & 0.71122 & 0.70413 \\ 
\bottomrule
\end{tabular}
\caption{Results of re-running Table 1 after fixing the NvFP bug.}
\end{table}




\begin{table}
    \centering
\begin{tabular}{c|c|cccccc}


Format & Transformation  &  PIQA & WinoGrande & HellaSwag & Arc-Easy & Arc-Challenge & Avg. \\ \midrule
‌Baseline  & - & 0.8074&0.7301 &0.7920 &0.7769 &0.5307 & 0.7274\\ \midrule

‌ \multirow{3}{*}{NVFP4}   & QuaRot & 0.7753&0.7167 & 0.7615& 0.7521& 0.4855& 0.6982 \\ 
                        & SpinQuant &0.7748  &0.7159 &0.7580 & 0.7428&0.4898 & 0.6962\\ 
                         & FlatQuant & & & & & & \\ \midrule
\multirow{3}{*}{MXFP4}  &    QuaRot & 0.7361&0.6796 &0.7253 &0.6456 &0.3968 & 0.6367 \\ 
                          &  SpinQuant & 0.7666& 0.6890& 0.7415& 0.67087& 0.4104& 0.6557\\ 
                         & FlatQuant & & & & & & \\ 

\bottomrule

\end{tabular}




\caption{Zero-shot accuracy   of using different trainable transformations on LLaMa3-8B model. }



\end{table}



